CrowdGenUI: Aligning LLM-Based UI Generation with Crowdsourced User Preferences

Large Language Models (LLMs) have demonstrated remarkable potential across various design domains, including user interface (UI) generation. However, current LLMs for UI generation tend to offer generic solutions that lack a nuanced understanding of task context and user preferences. We present CrowdGenUI, a framework that enhances LLM-based UI generation with crowdsourced user preferences. This framework addresses the limitations by guiding LLM reasoning with real user preferences, enabling the generation of UI widgets that reflect user needs and task-specific requirements. We evaluate our framework in the image editing domain by collecting a library of 720 user preferences from 50 participants, covering preferences such as predictability, efficiency, and explorability of various UI widgets. A user study (N=78) demonstrates that UIs generated with our preference-guided framework can better match user intentions compared to those generated by LLMs alone, highlighting the effectiveness of our proposed framework. We further discuss the study findings and present insights for future research on LLM-based user-centered UI generation.

==> commands_packages/dev-aliases.tex <==
%!TEX root = proceedings.tex

%%
%% Note: This file includes all new commands that are needed for the preliminary 
%% paper-writing (draft / review) stage of the paper. These commands should NOT
%% be included in the camera-ready version of the paper.
%%
%% All content in this file should be simple aliases (that take zero arguments). %% Custom commands with arguments should be provided in "dev-commands.tex".
%%

%% Note: Preprint notice to add to title when sharing early version of paper
\newcommand{\preprintNotice}{
    \textcolor{red}{
        Preprint: Currently under review. Please do not redistribute.}}

==> commands_packages/dev-commands.tex <==
%!TEX root = proceedings.tex

%%
%% Note: This file includes all new commands that are needed for the preliminary 
%% paper-writing (draft / review) stage of the paper. These commands should NOT
%% be included in the camera-ready version of the paper.
%%
%% All content in this file should take at least one argument. Custom commands 
%% for simple aliases should be provided in "dev-aliases.tex".
%%

%% Note: Custom colors for in-paper comments
\definecolor{LIGHTPINK}{RGB}{237,157,202}
\definecolor{LIGHTRED}{RGB}{210,121,121}
\definecolor{LIGHTORANGE}{RGB}{230,170,50}
\definecolor{LIGHTGOLD}{RGB}{210,194,121}
\definecolor{LIGHTGREEN}{RGB}{121,210,121}
\definecolor{LIGHTAQUA}{RGB}{121,206,210}
\definecolor{LIGHTBLUE}{RGB}{121,124,210}
\definecolor{LIGHTPURPLE}{RGB}{153,102,255}
\definecolor{RED}{RGB}{178,34,34}
\definecolor{GRAY}{RGB}{166,166,166}
\definecolor{WHITE}{RGB}{255,255,255}

%% Note: General TODO and cut commands
\newcommand{\todo}[1]{
    \addcontentsline{toc}{subsection}{  %
        \protect\numberline{}           % Align text appropriately
        \textcolor{RED}{[TODO] #1}}     % Add todo to the table of contents
    \textcolor{RED}{[TODO] \emph{#1}}}  % Typeset the todo note in the text
\newcommand{\cut}[1]{\textcolor{RED}{\st{#1}}}
\newcommand{\revise}[1]{\textcolor{blue}{#1}}

%%
%% Note: Labeled in-paper comments for collaborators (with and without underlined
%% text). Each author should specify a new command for their name with a
%% different comment color, using the example new command for \jane below. 
%% Alternatively, authors can use the more complicated \guest command, but must
%% provide their name each time they leave a comment.
%%

%% Usage: \yimeng[(OPTIONAL) Text to underline in square brackets]{Comment.}
\newcommandx{\yimeng}[2][1=] 
    {\setulcolor{LIGHTGREEN}{\ul{#1}} \textcolor{LIGHTGREEN}
    {[\textbf{Jane:} #2]}}
%% Usage: \guest[(OPTIONAL) Text to underline]{Name}{Comment text}
\newcommandx{\guest}[3][1=]
    {\setulcolor{LIGHTORANGE}{\ul{#1}} \textcolor{LIGHTORANGE} 
    {[\textbf{#2:} #3]}}

%%
%% Note: Custom status badges can be added to sections and subsections to label 
%% which ones are ready (or not) for feedback to facilitate collaboration amongst
%% authors. Badges should be added directly to the section heading.
%%
\newcommand{\badge}[2]{\colorbox{#1}{\small\textcolor{WHITE}{\texttt{#2}}}}
\newcommand{\headerBadge}[2]{\hspace*{\fill}\badge{#1}{#2}}

\newcommand{\locked}{\headerBadge{LIGHTPURPLE}{locked}}
\newcommand{\complete}{\headerBadge{LIGHTBLUE}{complete}}
\newcommand{\feedbackProvided}{\headerBadge{LIGHTGREEN}{feedback provided}}
\newcommand{\readyForFeedback}{\headerBadge{LIGHTORANGE}{feedback requested}}
\newcommand{\underRevision}{\headerBadge{LIGHTRED}{under revision}}
\newcommand{\incomplete}{\headerBadge{RED}{incomplete}}


% Define a new command for itemized lists with gray background highlight
\newcommand{\shadeditemize}[1]{
  \begingroup
  \color{gray}
  \begin{itemize}[label={\textcolor{gray}{$\bullet$}}]
    #1
  \end{itemize}
  \endgroup
}

\newcommand\circled[2][]{
\ifmmode
    \Circled[fill color=black,inner color=white, inner ysep=5pt, inner ysep=5pt, #1]{\mathsf{#2}}
    \else
    \Circled[fill color=white,inner color=black, inner ysep=5pt, inner ysep=5pt, #1]{\sffamily#2}
\fi
}

\newcommand{\wordcount}[1]{%
   \immediate\write18{texcount -1 -sum -merge #1.tex > #1.wc}%
    \vspace{1em} % Adds a line break and some vertical space above
    \hfill % Aligns the content to the right
    (\input{#1.wc} words) % Displays the word count from the file
    \vspace{1em} % Adds a line break and some vertical space below
}


==> commands_packages/dev-packages.tex <==
%!TEX root = proceedings.tex

%%
%% Note: This file includes all new packages that are needed for the preliminary 
%% paper-writing (draft / review) stage of the paper. These packages should NOT
%% be included in the camera-ready version of the paper. Each package should 
%% include a comment describing the purpose of the specific purpose of the new 
%% package for this submission.
%%
\usepackage{xargs}      % Used for new commands with optional arguments
\usepackage{soul}       % Used for custom comments
\usepackage{color}      % Used for custom colors in comments
\usepackage{xcolor}
\usepackage{enumitem}
\usepackage{soul}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{minted}
\usepackage{circledsteps}
% \usepackage{hyperref}

\usepackage{listings}
% Set up JSON style
\lstdefinelanguage{json}{
    basicstyle=\tiny\ttfamily,
    stepnumber=1,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    frame=none,
    literate=
     *{0}{{{\color{blue}0}}}{1}
      {1}{{{\color{blue}1}}}{1}
      {2}{{{\color{blue}2}}}{1}
      {3}{{{\color{blue}3}}}{1}
      {4}{{{\color{blue}4}}}{1}
      {5}{{{\color{blue}5}}}{1}
      {6}{{{\color{blue}6}}}{1}
      {7}{{{\color{blue}7}}}{1}
      {8}{{{\color{blue}8}}}{1}
      {9}{{{\color{blue}9}}}{1}
      {:}{{{\color{black}:}}}{1}
      {,}{{{\color{black},}}}{1}
      {\{}{{{\color{orange}\{}}}{1}
      {\}}{{{\color{orange}\}}}}{1}
      {[}{{{\color{orange}[}}}{1}
      {]}{{{\color{orange}]}}}{1},
}
% Set up Python code style
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}  % RGB value for dark green
\lstset{
    language=Python,              % Set language to Python
    basicstyle=\tiny\ttfamily,         % Code font (monospaced)
    keywordstyle=\color{blue},    % Keywords in blue
    stringstyle=\color{red},      % Strings in red
    commentstyle=\color{darkgreen},    % Comments in gray
    numberstyle=\tiny\color{gray},% Line number style
    stepnumber=1,                 % Step for line numbering
    numbersep=8pt,                % Distance between line numbers and code
    showstringspaces=false,       % Don't show spaces in strings
    breaklines=true,              % Automatic line breaking
    frame=none,                   % No borders around the code block
    tabsize=4,                    % Set tab width to 4 spaces
}

% Define custom style for Markdown
\lstdefinelanguage{markdown}{
    basicstyle=\tiny\ttfamily,
    morekeywords={\#, \*\*, \*, -}, % Escape special characters
    keywordstyle=\color{blue},
    sensitive=false,
    morecomment=[l]{>}, % Define blockquotes
    commentstyle=\color{gray}\itshape,
    morestring=[b]"
}


==> commands_packages/published-aliases.tex <==
%!TEX root = proceedings.tex

%%
%% Note: This file includes all custom new commands that are needed for the 
%% final, camera-ready version of the paper. All content in this file should 
%% not take any arguments. Custom commands with arguments should be provided in 
%% "published-commands.tex".
%%

%% Note: New command for referencing (and easily changing) the system name
\newcommand{\sys}{StillUndecided}

%% Note: Commands for spacing Latin letters/abbreviations
\newcommand{\ie}{{i.e.,}\xspace}
\newcommand{\eg}{{e.g.,}\xspace}
\newcommand{\etal}{{et~al\xperiod}\xspace}
\newcommand{\aka}{{a.k.a.}\xspace}
\newcommand{\etc}{{etc\xperiod}\xspace}

==> commands_packages/published-commands.tex <==
%!TEX root = proceedings.tex

%%
%% Note: This file includes all custom new commands that are needed for the 
%% final, camera-ready version of the paper. All content in this file should 
%% take at least one argument. Custom commands for simple aliases should be
%% provided in "published-aliases.tex".
%%

%% Note: Custom new commands for styling participant quotes.
\newcommand{\myquote}[1]{\emph{``#1''}} % Italic text in quotation marks
\newcommand{\myquoteparticipant}[2]{    % \myquote WITH P# and non-breaking space
    \myquote{#1}~(#2)}
\newcommand{\mylongquote}[1]{           % Italic block quote, no quotation marks or P#
    \begin{quote}\emph{#1}\end{quote}}

%% Note: Commands for custom styling of bold, inline paragraph headings
\newcommand{\parHeading}[1]{\vspace{8px}\noindent{\textbf{#1}}}


==> commands_packages/published-packages.tex <==
%!TEX root = proceedings.tex

%%
%% Note: This file includes all new packages that are needed for the final, 
%% camera-ready version of the paper. It is important to ensure that all packages
%% included in this file are approved by the conference's submission process.
%% Each package should include a comment describing the purpose of the specific
%% purpose of the new package for this submission.
%%
\usepackage{xspace}     % Used for abbreviation spacing
\usepackage{xpunctuate} % Used for abbreviation spacing

==> figures/crowdsourcing_image_adjust_hue.tex <==

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.95\textwidth}
        \includegraphics[width=\textwidth]{figures/crowdsourcing_ui/crowdsourcing_image_adjust_hue.png}
        \caption{UI widget interaction.}
    \end{subfigure}
    \par\vspace{0.5cm}
    \begin{subfigure}[b]{0.95\textwidth}
        \includegraphics[width=\textwidth]{figures/crowdsourcing_ui/crowdsourcing_image_adjust_hue_selector.png}
        \caption{UI widget preference selection.}
    \end{subfigure}
    \caption{Crowdsourcing user interface for task: adjusting image hue.}
    \label{fig:ui_image_adjust_hue}
\end{figure}


==> figures/crowdsourcing_image_place_watermark.tex <==

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/crowdsourcing_ui/crowdsourcing_image_place_watermark.png}
    \caption{User interface for task: placing a watermark on an image.}
    \label{fig:ui_image_place_watermark}
\end{figure}


==> figures/reasoning_ml_signal_tasks.tex <==

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/reasoning_widget_distribution/reasoning_signal_adjust_quantization.pdf}
    \caption{Reasoned UI widgets for \texttt{signal\_adjust\_quantization\_level} generated by LLMs with three sizes of the crowdsourced libraries and without any library.}
    \label{fig:reasoning_signal_adjust_quantization}
\end{figure}


==> figures/user_eval_design_align_text.tex <==

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.95\textwidth}
        \includegraphics[width=\textwidth]{figures/user_eval_ui/user_eval_design_align_text.png}
        \caption{UI widget interaction.}
        \label{fig:ui_design_align_text_widget_interaction}
    \end{subfigure}
    \par\vspace{0.5cm}
    \begin{subfigure}[b]{0.95\textwidth}
        \includegraphics[width=\textwidth]{figures/user_eval_ui/user_eval_design_align_text_selector.png}
        \caption{Pairwise comparison preference selection.}
        \label{fig:ui_design_align_text_preference_selection}
    \end{subfigure}
    \caption{User evaluation user interface for task: \texttt{design\_align\_text}.}
    \label{fig:ui_design_align_text}
\end{figure}


==> figures/violin_plot.tex <==

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/user_eval_selection_distribution_across_tasks/violin_plot_predictability.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/user_eval_selection_distribution_across_tasks/violin_plot_efficiency.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/user_eval_selection_distribution_across_tasks/violin_plot_explorability.pdf}
    \end{subfigure}
    \caption{Distribution of user preference selection counts of three preference aspects across all tasks.}
    \label{fig:user_eval_per_aspect_violin}
\end{figure}


==> sections/acknowledgements.tex <==

\begin{acks}

\end{acks}


==> sections/header.tex <==
%!TEX root = proceedings.tex

%% NOTE: These files include necessary content for the final, camera-ready paper
\input{commands_packages/published-packages} % New (approved) packages
\input{commands_packages/published-aliases}  % Custom command aliases
\input{commands_packages/published-commands} % Custom commands / styling

%% NOTE: These files include content that is useful for paper-writing and should
%% be excluded from the final, camera-ready paper by commenting them out.
\input{commands_packages/dev-packages} % New packages for custom comments
\input{commands_packages/dev-aliases}  % Custom command aliases for draft/review
\input{commands_packages/dev-commands} % Custom commands / styling / comments
